Innovation Modeling Grid

This technical document presents the committee driven innovation modeling methodology "Innovation Modeling Grid" in detail. This document is the successor of three publications on IMoG and focuses on presenting all details of the methodology

==> content/content_outline.tex <==
\begin{enumerate}
	\item Motivation:
	\item IMoG Process
	\item Methodology Overview
	\begin{itemize}
		\item 
		\item handlungsempfehlungen hinzufügen
	\end{itemize}
	\item[3b)] Excurs on design principles
	\item[3c)] Excurs on glossary
	\item[3d)] E-Scooter example
	\item[4-10)] Each process step (including each Perspective (Model Elements + Example))
	\item[11.] Inter Perspective view (Excurs on Decomposition / Refinement)
	\item[12.] Tooling Example / Current State
	\item[13.] Evaluation
	\item[14.] Conclusion and Future Work (No future work)
\end{enumerate}

